Remembering Chandra Kintala

With this contribution we would like to remember Chandra M. R. Kintala who passed away in November 2009. We will give short overviews of his CV and his contributions to the field of theoretical and applied computer science and, given the opportunity, will attempt to present the current state of limited nondeterminism and limited resources for machines. Finally, we will briefly touch on some research topics which hopefully will be addressed in the not so distant future.

==> eptcsdata.tex <==
\providecommand{\firstpage}{15}
\providecommand{\publicationstatus}{I. McQuillan and G. Pighizzini (Eds.): 12th International Workshop\\on Descriptional Complexity of Formal Systems (DCFS 2010)\\
EPTCS 31, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.31.4}{10.4204/EPTCS.31.4}}

